The evolution of the radio luminosity function of group galaxies in COSMOS

[Abridged] To understand the role of the galaxy group environment on galaxy evolution, we present a study of radio luminosity functions (RLFs) of group galaxies based on the VLA-COSMOS 3 GHz Large Project. The radio-selected sample of 7826 COSMOS galaxies with robust optical/near-infrared counterparts, excellent photometric coverage, and the COSMOS X-ray galaxy groups (M_200c > 10^13.5 M_sun) enables us to construct the RLF of group galaxies (GGs) and their contribution to the total RLF since z ~ 2.3. Using the Markov chain Monte Carlo algorithm, we fit a redshift-dependent pure luminosity evolution model and a linear and power-law model to the luminosity functions. We compare it with past RLF studies from VLA-COSMOS on individual populations of radio-selected star-forming galaxies (SFGs) and galaxies hosting active galactic nuclei (AGN). These populations are classified based on the presence or absence of a radio excess concerning the star-formation rates derived from the infrared emission. We find that the density of radio galaxies in groups is low compared to the field at z ~ 2 down to z ~ 1.25, followed by a sharp increase at z ~ 1 by a factor of 6, and then a smooth decline towards low redshifts. This trend is caused by both decrease in the volume abundance of massive groups at high-z and the changes in the halo occupation of radio AGN, which are found by other studies to reside at smaller halo mass groups. This indicates that the bulk of high-$z$ log10(M_200c/M_sun) > 13.5 groups must have been forming recently, and so the cooling has not been established as yet. The slope of the GG RLF is flatter compared to the field, with excess at high radio luminosities. The evolution in the GG RLF is driven mainly by satellite galaxies in groups. A drop in occurrence of AGN in groups at z > 1 by a factor of 6, manifests an important detail on the processes governing galaxy evolution.

==> figures/radioprops_ggs.tex <==
29  &  79  &  150.447297  &  2.053936  &  150.4456  &  2.054150  &  0.323  &  0.324 $^{ s }$  &  24.36  &  1.81 $\pm$ 0.86  &  1.73 $\pm$ 0.58  &  -1.38  &  0  & AGN \\ 
35  &  333  &  150.042302  &  2.694820  &  150.04736  &  2.693170  &  0.218  &  0.219 $^{ s }$  &  23.50  &  1.03 $\pm$ 0.40  &  1.26 $\pm$ 0.43  &  -1.40  &  0  & AGN \\ 
42  &  11  &  150.185632  &  1.661683  &  150.19728  &  1.658950  &  0.221  &  0.220 $^{ s }$  &  23.34  &  2.54 $\pm$ 0.75  &  2.23 $\pm$ 0.24  &  -1.08  &  5  & AGN \\ 
44  &  237  &  150.110399  &  2.708261  &  150.11756  &  2.692520  &  0.351  &  0.349 $^{ s }$  &  24.48  &  2.19 $\pm$ 0.95  &  1.96 $\pm$ 0.52  &  -1.33  &  2  & AGN \\ 
45  &  189  &  149.905915  &  2.396440  &  149.91816  &  2.388030  &  0.742  &  0.736 $^{ s }$  &  24.40  &  1.82 $\pm$ 1.30  &  1.58 $\pm$ 0.85  &  -1.68  &  3  & AGN \\ 
61  &  134  &  149.649621  &  2.209249  &  149.6507  &  2.211630  &  0.954  &  0.951 $^{ s }$  &  23.85  &  2.27 $\pm$ 1.58  &  1.78 $\pm$ 0.88  &  -1.69  &  0  & AGN \\ 
80  &  264  &  149.998389  &  2.769141  &  149.99834  &  2.774410  &  0.166  &  0.165 $^{ s }$  &  23.54  &  1.03 $\pm$ 0.45  &  1.28 $\pm$ 0.48  &  -1.29  &  0  & AGN \\ 
88  &  52  &  150.44703  &  1.882829  &  150.44759  &  1.883190  &  0.670  &  0.672 $^{ s }$  &  24.02  &  1.84 $\pm$ 1.17  &  1.62 $\pm$ 0.74  &  -1.65  &  0  & AGN \\ 
99  &  25  &  149.884002  &  1.750996  &  149.85402  &  1.770230  &  0.122  &  0.124 $^{ s }$  &  22.10  &  1.58 $\pm$ 0.08  &  1.65 $\pm$ -0.05  &  -1.05  &  0  & AGN \\ 
103  &  143  &  150.207423  &  2.281893  &  150.22014  &  2.278510  &  0.917  &  0.885 $^{ s }$  &  24.53  &  2.18 $\pm$ 1.43  &  1.75 $\pm$ 0.79  &  -1.68  &  3  & AGN \\ 
119  &  245  &  150.695821  &  2.760741  &  150.69144  &  2.754350  &  0.630  &  0.646 $^{ s }$  &  23.36  &  2.05 $\pm$ 1.34  &  1.76 $\pm$ 0.84  &  -1.59  &  2  & AGN \\ 
127  &  187  &  149.623522  &  2.399203  &  149.62376  &  2.399380  &  0.846  &  0.840 $^{ s }$  &  24.10  &  2.33 $\pm$ 1.60  &  1.86 $\pm$ 0.92  &  -1.64  &  0  & AGN \\ 
149  &  44  &  149.805372  &  1.874522  &  149.79852  &  1.872330  &  1.329  &  1.350 $^{ p }$  &  25.10  &  2.40 $\pm$ 1.98  &  1.71 $\pm$ 1.07  &  -1.81  &  0  & AGN \\ 
156  &  217  &  150.007104  &  2.453454  &  150.0037  &  2.454870  &  0.731  &  0.732 $^{ s }$  &  24.14  &  1.73 $\pm$ 1.15  &  1.52 $\pm$ 0.73  &  -1.71  &  0  & AGN \\ 
178  &  46  &  150.250884  &  1.863985  &  150.24614  &  1.865000  &  0.530  &  0.529 $^{ s }$  &  23.81  &  1.61 $\pm$ 1.01  &  1.52 $\pm$ 0.71  &  -1.61  &  0  & AGN \\ 
182  &  190  &  149.441577  &  2.425937  &  149.45692  &  2.433530  &  0.481  &  0.484 $^{ s }$  &  24.03  &  2.16 $\pm$ 1.36  &  1.89 $\pm$ 0.89  &  -1.46  &  0  & AGN \\ 
183  &  149  &  150.415664  &  2.430186  &  150.42235  &  2.428000  &  0.124  &  0.124 $^{ s }$  &  22.34  &  1.81 $\pm$ 0.16  &  1.79 $\pm$ -0.06  &  -1.01  &  0  & AGN \\ 
187  &  311  &  149.942948  &  2.600608  &  149.93887  &  2.606860  &  0.344  &  0.342 $^{ s }$  &  24.84  &  1.50 $\pm$ 0.56  &  1.52 $\pm$ 0.38  &  -1.47  &  2  & AGN \\ 
203  &  291  &  149.478815  &  2.521843  &  149.48956  &  2.516580  &  0.092  &  0.092 $^{ s }$  &  22.10  &  0.83 $\pm$ 0.12  &  1.17 $\pm$ 0.26  &  -1.09  &  84  & SFG \\ 
211  &  215  &  150.172574  &  2.523342  &  150.17097  &  2.523630  &  0.697  &  0.697 $^{ s }$  &  24.14  &  1.58 $\pm$ 1.13  &  1.44 $\pm$ 0.77  &  -1.72  &  1  & AGN \\ 
213  &  24  &  150.30117  &  1.689921  &  150.29169  &  1.689350  &  0.530  &  0.527 $^{ s }$  &  24.14  &  1.88 $\pm$ 1.02  &  1.70 $\pm$ 0.63  &  -1.55  &  1  & AGN \\ 
220  &  203  &  149.666143  &  2.474287  &  149.65762  &  2.479720  &  0.956  &  0.948 $^{ s }$  &  23.50  &  2.28 $\pm$ 1.59  &  1.78 $\pm$ 0.89  &  -1.70  &  2  & SFG \\ 
226  &  36  &  149.894896  &  1.764946  &  149.89491  &  1.764970  &  0.530  &  0.531 $^{ s }$  &  23.34  &  1.76 $\pm$ 1.09  &  1.61 $\pm$ 0.74  &  -1.58  &  1  & AGN \\ 
235  &  20  &  150.325431  &  1.607013  &  150.32584  &  1.605100  &  0.222  &  0.227 $^{ s }$  &  23.01  &  1.13 $\pm$ 0.43  &  1.33 $\pm$ 0.42  &  -1.38  &  8  & AGN \\ 
246  &  126  &  150.750943  &  2.199992  &  150.74525  &  2.196520  &  0.372  &  0.372 $^{ s }$  &  23.93  &  1.68 $\pm$ 0.99  &  1.62 $\pm$ 0.72  &  -1.46  &  0  & SFG \\ 
251  &  173  &  150.058047  &  2.380425  &  150.05441  &  2.374090  &  0.347  &  0.347 $^{ s }$  &  22.63  &  1.37 $\pm$ 0.66  &  1.44 $\pm$ 0.51  &  -1.50  &  1  & AGN \\ 
261  &  271  &  149.91793  &  2.701673  &  149.91853  &  2.700660  &  0.891  &  0.890 $^{ s }$  &  24.22  &  2.33 $\pm$ 1.60  &  1.84 $\pm$ 0.90  &  -1.66  &  4  & AGN \\ 
278  &  302  &  150.090688  &  2.205629  &  150.09077  &  2.205680  &  0.426  &  0.427 $^{ s }$  &  23.37  &  1.01 $\pm$ 0.63  &  1.18 $\pm$ 0.57  &  -1.66  &  0  & AGN \\ 
279  &  221  &  150.565828  &  2.496444  &  150.57024  &  2.498640  &  1.146  &  1.147 $^{ s }$  &  23.58  &  2.42 $\pm$ 2.01  &  1.80 $\pm$ 1.17  &  -1.74  &  0  & AGN \\ 
302  &  14  &  150.247725  &  1.542408  &  150.24973  &  1.543310  &  0.886  &  0.886 $^{ p }$  &  24.21  &  2.50 $\pm$ 1.88  &  1.88 $\pm$ 1.06  &  -1.69  &  0  & AGN \\ 

